A new benchmark for group distribution shifts in hand grasp regression for object manipulation. Can meta-learning raise the bar?

Understanding hand-object pose with computer vision opens the door to new applications in mixed reality, assisted living or human-robot interaction. Most methods are trained and evaluated on balanced datasets. This is of limited use in real-world applications; how do these methods perform in the wild on unknown objects? We propose a novel benchmark for object group distribution shifts in hand and object pose regression. We then test the hypothesis that meta-learning a baseline pose regression neural network can adapt to these shifts and generalize better to unknown objects. Our results show measurable improvements over the baseline, depending on the amount of prior knowledge. For the task of joint hand-object pose regression, we observe optimization interference for the meta-learner. To address this issue and improve the method further, we provide a comprehensive analysis which should serve as a basis for future work on this benchmark.

==> fig/linear_regression.tex <==
\begin{figure}[tb]
    \centering
    \begin{subfigure}[t]{0.5\textwidth}
        \begin{center}
        \includegraphics[width=\textwidth]{fig/handonly_conditioned_regression.pdf}
        \label{fig:exp1_regression}
        \caption{\textbf{Experiment 1} -- Regression.}
        \end{center}
    \end{subfigure}
    \begin{subfigure}[t]{0.5\textwidth}
        \begin{center}
            \includegraphics[width=\textwidth]{fig/handobj_conditioned_regression.pdf}
            \label{fig:exp1_regression}
            \caption{\textbf{Experiment 2} -- Regression.}
        \end{center}
    \end{subfigure}
    \label{fig:regression}
    \caption{\textbf{Linear regression} -- }
\end{figure}

==> sec/2_related.tex <==
% \input{fig/overview} %< bloody latex and its heuristics for figure placement
\section{Related works}
\label{sec:related}
The problem of joint hand-object pose has been addressed in several ways, but rarely as optimising for the generalisability to
unknown objects. To the best of our knowledge, this has only been measured in the HANDS 2019 public challenge \citep{Armagan2020MeasuringGT} and
in \citep{Yu2022HandOAH}, although grasp synthesis of unknown objects is demonstrated in \citep{Karunratanakul2020GraspingFL}.
Meta-learning has been used to adapt to unobserved targets in regression \citep{Park2019FewShotAG,Xiao2020OnlineMA,Park2018MetaTrackerFA},
however other approaches are used for test-time adaptation.

% TODO: Rename to hand grasp prediction?
\paragraph{Hand-Object Pose Estimation (HOPE)}
Novel methods have been proposed, such as \citep{Cheng2021Semisupervised3H} with a pose dictionary
module to learn with limited data in a semi-supervised fashion, which yields more robust
predictions than SOTA deep learning architectures trained on fully-labelled data, although it is
not evaluated on unknown objects. Akin to this method, \citep{Li2021ArtiBoostBA} propose a novel
online data enrichment strategy for articulated hand-object pose prediction which allows a baseline
to outperform the state of the art. It explores the pose space via optimised sample synthesis to
enrich the data, thus making it model-agnostic, however, this only takes effect at training time,
hence not allowing adaptation to unknown objects. \citep{Yang2020CPFLA} introduce an explicit
hand-object contact representation, called \textit{Contact Potential Field}, as a spring-mass
system for plausible grasps. They demonstrate state-of-the-art reconstruction of hand-object
interaction with less mesh penetration and more physically realistic grasps, but their method
requires the object mesh as prior. 
%This limits the applicability of the method.
Similarly, \citep{Karunratanakul2020GraspingFL} propose an implicit representation of hand-object
pose as a Signed Distance Field (SDF) in a joint function space, which they use to reconstruct
poses of previously seen objects or synthesise grasps of unseen ones. Hand-object pose estimation
for unseen objects is demonstrated in \citep{Yu2022HandOAH} through self-supervision for test-time
optimisation of hand and object SDFs. They achieve arguably better results than
\citep{Karunratanakul2020GraspingFL} but require known camera parameters.

\paragraph{Meta-Learning}
Meta-Learning is typically applied in the few-shot classification scenario, although some methods
are applied to regression problems. For the latter, three main categories: optimisation-based
methods, memory-based methods, and lastly generative models for functions (see
\citep{Hospedales2021MetaLearningIN} and \citep{Huisman2021ASO} for an overview). Optimisation-based
methods \citep{andrychowicz_learning_2016} used an LSTM to learn the update rule of a learner
network. Later, inner-loop-based methods were introduced by MAML \citep{maml} which removes extra
parameters and learns a good initialisation for the learner to quickly adapt to novel tasks via
second-order gradient descent. Improvements were proposed by \citep{Antoniou} regarding the
instability and generalisation. \citep{ANIL} analysed the extent to which MAML only
reuses learnt features and proposed to apply inner-loop optimisation on the head of a CNN only.
Generalisation was improved by \citep{Rusu2019MetaLearningWL} via latent embedding
optimisation, at a high computational cost, while \citep{Nichol2018ReptileAS} tackled the
first-order version of MAML to improve its computational cost and generalisation.
A different paradigm is memory-based methods
\citep{Santoro2016OneshotLW,Santoro2016MetaLearningWM} which adopt a strategy closer to human-like
learning by storing representations of concepts in modifiable memory cells.
%\citep{Mishra2018ASN} improved upon this concept using the attention mechanism and yielding
%state-of-the-art results on image classification and regression tasks.
Neural Processes \citep{Garnelo2018ConditionalNP,Garnelo2018NeuralP,Kim2019AttentiveNP},
introduced as a blend between Gaussian Processes and Neural Networks, model uncertainty. They are
especially suited to regression problems by meta-learning functions from sets of observations,
similarly to \citep{Edwards2017TowardsAN,Bachman2018VFuncAD}. However, by using latent space
aggregations they tend to underfit the
context for high-dimensional tasks. This is underlined by \citep{Sitzmann2020MetaSDFMS} proposing to
meta-learn an SDF for implicit shape
representation using MAML. % This concerns the follow-up
%experiment, but I may keep it for the analysis (or simply move this to the analysis, although I already refer to it!).

\paragraph{Test-time adaptation}
Broadly speaking, this area relates to methods that enhance a model's performance on a specific
case at test time. This was explored using meta-learning in \citep{Gui2018FewShotHM} for human
motion prediction, with a specialisation of MAML significantly outperforming the original on this
problem. \citep{Park2018MetaTrackerFA} derived a meta-learning algorithm for online object tracking,
with state-of-the-art accuracy. Similarly, \citep{Xiao2020OnlineMA} propose an inner-loop-based
meta-leaner for video object segmentation which greatly outperforms a baseline in accuracy and
fine-tuning time. \citep{Park2019FewShotAG} directly applied MAML on gaze estimation to train
person-specific models with few examples and outperform existing methods. Other methods
\citep{Sun2020TestTimeTW,Hao2021TestTimePW}  use a regular training stage but adopt an online
adaptation strategy for new test-cases, which implies defining appropriate self-supervision
objectives. Test-time adaptation has been applied to single-view mesh reconstruction for
in-the-wild videos in \citep{Li2020OnlineAF} using self-supervision and temporal consistency.
Recently, in single-view mesh reconstruction, \citep{Michalkiewicz2020FewShotS3,Yang2021SingleView3O,Wallace2019FewShotGF}
investigate the use of learnt object priors and propose
different methods for inferring new priors on unknown objects.
%In this work, we apply meta-learning
%to hand grasp prediction, a sub-problem of HOPE, in order to achieve test-time adaptation to unseen
%objects.


==> tab/dexycb.tex <==
\begin{table}[h!]
\centering
    \begin{tabular}{ |c|p{3.2cm}||c|c|  }
        \hline
        Method & \# objects & MSE & MAE \\
        \hline
        ANIL & 1 & & \\
        Baseline & 1 &  & \\
        \hline
        ANIL & 2 & & \\
        Baseline & 2 &  & \\
        \hline
        ANIL & 3 & & \\
        Baseline & 3 &  & \\
        \hline
        ANIL & 4 & & \\
        Baseline & 4 &  & \\
        \hline
        ANIL & 5 & & \\
        Baseline & 5 &  & \\
        \hline
        ANIL & 6 & & \\
        Baseline & 6 &  & \\
        \hline
        ANIL & 7 & & \\
        Baseline & 7 &  & \\
        \hline
        ANIL & 8 & & \\
        Baseline & 8 &  & \\
        \hline
        ANIL & 9 & & \\
        Baseline & 9 &  & \\
        \hline
        ANIL & 10 & & \\
        Baseline & 10 &  & \\
        \hline
        ANIL & 11 & 873.35 & 21.95\\
        Baseline & 11 &  & \\
        \hline
        ANIL & 12 & 897.32 & 22.29\\
        Baseline & 12 &  & \\
        \hline
        ANIL & 13 & 1014.09 & 24.07\\
        Baseline & 13 &  & \\
        \hline
    \end{tabular}
    \caption{Evaluation on DexYCB. ResNet-18 is used, and for ANIL, $k=10$, $q=50$ and $15$ adaptation steps are used.
    The best of 5 runs for ANIL is used, since it is stochastic at test time. The baseline consistently performs better than ANIL,
    although ANIL shows a non-consistent increase in MSE.}
    \label{table:dexycb}
\end{table}

==> tab/procrustes/affinity_mat.tex <==
% \usepackage{rotating}
% \usepackage{array}
% \usepackage{booktabs}
% \usepackage{vcell}
% \usepackage{colortbl}


\begin{table}
\centering
\arrayrulecolor[rgb]{0.502,0.502,0.502}
\begin{tabular}{!{\color{black}\vrule}>{\hspace{0pt}}m{0.033\linewidth}!{\color{black}\vrule}>{\hspace{0pt}}m{0.041\linewidth}|>{\hspace{0pt}}m{0.036\linewidth}|>{\hspace{0pt}}m{0.036\linewidth}|>{\hspace{0pt}}m{0.05\linewidth}|>{\hspace{0pt}}m{0.041\linewidth}|>{\hspace{0pt}}m{0.043\linewidth}|>{\hspace{0pt}}m{0.036\linewidth}|>{\hspace{0pt}}m{0.038\linewidth}|>{\hspace{0pt}}m{0.05\linewidth}|>{\hspace{0pt}}m{0.029\linewidth}|>{\hspace{0pt}}m{0.036\linewidth}|>{\hspace{0pt}}m{0.036\linewidth}|>{\hspace{0pt}}m{0.033\linewidth}|>{\hspace{0pt}}m{0.035\linewidth}|>{\hspace{0pt}}m{0.04\linewidth}|>{\hspace{0pt}}m{0.041\linewidth}|>{\hspace{0pt}}m{0.029\linewidth}|>{\hspace{0pt}}m{0.043\linewidth}|>{\hspace{0pt}}m{0.05\linewidth}|>{\hspace{0pt}}m{0.035\linewidth}!{\color{black}\vrule width \lightrulewidth}} 
\arrayrulecolor{black}\cline{2-21}
\multicolumn{1}{>{\hspace{0pt}}p{0.033\linewidth}!{\color{black}\vrule}}{\vcell{\begin{sideways}\end{sideways}}} & \multicolumn{1}{>{\hspace{0pt}}p{0.041\linewidth}|}{\vcell{\begin{sideways}Master chef can\end{sideways}}} & \multicolumn{1}{>{\hspace{0pt}}p{0.036\linewidth}|}{\vcell{\begin{sideways}Cracker box\end{sideways}}} & \multicolumn{1}{>{\hspace{0pt}}p{0.036\linewidth}|}{\vcell{\begin{sideways}Sugar box\end{sideways}}} & \multicolumn{1}{>{\hspace{0pt}}p{0.05\linewidth}|}{\vcell{\begin{sideways}Tomato soup can\end{sideways}}} & \multicolumn{1}{>{\hspace{0pt}}p{0.041\linewidth}|}{\vcell{\begin{sideways}Mustard bottle\end{sideways}}} & \multicolumn{1}{>{\hspace{0pt}}p{0.043\linewidth}|}{\vcell{\begin{sideways}Tuna fish can\end{sideways}}} & \multicolumn{1}{>{\hspace{0pt}}p{0.036\linewidth}|}{\vcell{\begin{sideways}Pudding box\end{sideways}}} & \multicolumn{1}{>{\hspace{0pt}}p{0.038\linewidth}|}{\vcell{\begin{sideways}Gelatin box\end{sideways}}} & \multicolumn{1}{>{\hspace{0pt}}p{0.05\linewidth}|}{\vcell{\begin{sideways}Potted meat can\end{sideways}}} & \multicolumn{1}{>{\hspace{0pt}}p{0.029\linewidth}|}{\vcell{\begin{sideways}Banana\end{sideways}}} & \multicolumn{1}{>{\hspace{0pt}}p{0.036\linewidth}|}{\vcell{\begin{sideways}Pitcher base\end{sideways}}} & \multicolumn{1}{>{\hspace{0pt}}p{0.036\linewidth}|}{\vcell{\begin{sideways}Bleach cleanser\end{sideways}}} & \multicolumn{1}{>{\hspace{0pt}}p{0.033\linewidth}|}{\vcell{\begin{sideways}Bowl\end{sideways}}} & \multicolumn{1}{>{\hspace{0pt}}p{0.035\linewidth}|}{\vcell{\begin{sideways}Mug\end{sideways}}} & \multicolumn{1}{>{\hspace{0pt}}p{0.04\linewidth}|}{\vcell{\begin{sideways}Power drill\end{sideways}}} & \multicolumn{1}{>{\hspace{0pt}}p{0.041\linewidth}|}{\vcell{\begin{sideways}Wood block\end{sideways}}} & \multicolumn{1}{>{\hspace{0pt}}p{0.029\linewidth}|}{\vcell{\begin{sideways}Scissors\end{sideways}}} & \multicolumn{1}{>{\hspace{0pt}}p{0.043\linewidth}|}{\vcell{\begin{sideways}Large marker\end{sideways}}} & \multicolumn{1}{>{\hspace{0pt}}p{0.05\linewidth}|}{\vcell{\begin{sideways}Extra large clamp\end{sideways}}} & \multicolumn{1}{>{\hspace{0pt}}p{0.035\linewidth}!{\color{black}\vrule width \lightrulewidth}}{\vcell{\begin{sideways}Foam brick\end{sideways}}}  \\[-\rowheight]
\multicolumn{1}{>{\hspace{0pt}}m{0.033\linewidth}!{\color{black}\vrule}}{\printcellmiddle}                       & \multicolumn{1}{>{\hspace{0pt}}m{0.041\linewidth}|}{\printcelltop}                                         & \multicolumn{1}{>{\hspace{0pt}}m{0.036\linewidth}|}{\printcellmiddle}                                  & \multicolumn{1}{>{\hspace{0pt}}m{0.036\linewidth}|}{\printcellmiddle}                                & \multicolumn{1}{>{\hspace{0pt}}m{0.05\linewidth}|}{\printcellmiddle}                                      & \multicolumn{1}{>{\hspace{0pt}}m{0.041\linewidth}|}{\printcellmiddle}                                     & \multicolumn{1}{>{\hspace{0pt}}m{0.043\linewidth}|}{\printcellmiddle}                                    & \multicolumn{1}{>{\hspace{0pt}}m{0.036\linewidth}|}{\printcellmiddle}                                  & \multicolumn{1}{>{\hspace{0pt}}m{0.038\linewidth}|}{\printcellmiddle}                                  & \multicolumn{1}{>{\hspace{0pt}}m{0.05\linewidth}|}{\printcellmiddle}                                      & \multicolumn{1}{>{\hspace{0pt}}m{0.029\linewidth}|}{\printcellmiddle}                             & \multicolumn{1}{>{\hspace{0pt}}m{0.036\linewidth}|}{\printcellmiddle}                                   & \multicolumn{1}{>{\hspace{0pt}}m{0.036\linewidth}|}{\printcellmiddle}                                      & \multicolumn{1}{>{\hspace{0pt}}m{0.033\linewidth}|}{\printcellmiddle}                           & \multicolumn{1}{>{\hspace{0pt}}m{0.035\linewidth}|}{\printcellmiddle}                          & \multicolumn{1}{>{\hspace{0pt}}m{0.04\linewidth}|}{\printcellmiddle}                                  & \multicolumn{1}{>{\hspace{0pt}}m{0.041\linewidth}|}{\printcellmiddle}                                 & \multicolumn{1}{>{\hspace{0pt}}m{0.029\linewidth}|}{\printcellmiddle}                               & \multicolumn{1}{>{\hspace{0pt}}m{0.043\linewidth}|}{\printcellmiddle}                                   & \multicolumn{1}{>{\hspace{0pt}}m{0.05\linewidth}|}{\printcellmiddle}                                        & \multicolumn{1}{>{\hspace{0pt}}m{0.035\linewidth}!{\color{black}\vrule width \lightrulewidth}}{\printcellmiddle}                                  \\ 
\hline
Master chef can                                                                                                  & 0                                                                                                          &                                                                                                        &                                                                                                      &                                                                                                           &                                                                                                           &                                                                                                          &                                                                                                        &                                                                                                        &                                                                                                           &                                                                                                   &                                                                                                         &                                                                                                            &                                                                                                 &                                                                                                &                                                                                                       &                                                                                                       &                                                                                                     &                                                                                                         &                                                                                                             &                                                                                                                                                   \\ 
\arrayrulecolor[rgb]{0.502,0.502,0.502}\hline
Cracker box                                                                                                      &                                                                                                            & 0                                                                                                      &                                                                                                      &                                                                                                           &                                                                                                           &                                                                                                          &                                                                                                        &                                                                                                        &                                                                                                           &                                                                                                   &                                                                                                         &                                                                                                            &                                                                                                 &                                                                                                &                                                                                                       &                                                                                                       &                                                                                                     &                                                                                                         &                                                                                                             &                                                                                                                                                   \\ 
\hline
Sugar box                                                                                                        &                                                                                                            &                                                                                                        & 0                                                                                                    &                                                                                                           &                                                                                                           &                                                                                                          &                                                                                                        &                                                                                                        &                                                                                                           &                                                                                                   &                                                                                                         &                                                                                                            &                                                                                                 &                                                                                                &                                                                                                       &                                                                                                       &                                                                                                     &                                                                                                         &                                                                                                             &                                                                                                                                                   \\ 
\hline
Tomato soup can                                                                                                  &                                                                                                            &                                                                                                        &                                                                                                      & 0                                                                                                         &                                                                                                           &                                                                                                          &                                                                                                        &                                                                                                        &                                                                                                           &                                                                                                   &                                                                                                         &                                                                                                            &                                                                                                 &                                                                                                &                                                                                                       &                                                                                                       &                                                                                                     &                                                                                                         &                                                                                                             &                                                                                                                                                   \\ 
\hline
Mustard bottle                                                                                                   &                                                                                                            &                                                                                                        &                                                                                                      &                                                                                                           & 0                                                                                                         &                                                                                                          &                                                                                                        &                                                                                                        &                                                                                                           &                                                                                                   &                                                                                                         &                                                                                                            &                                                                                                 &                                                                                                &                                                                                                       &                                                                                                       &                                                                                                     &                                                                                                         &                                                                                                             &                                                                                                                                                   \\ 
\hline
Tuna fish can                                                                                                    &                                                                                                            &                                                                                                        &                                                                                                      &                                                                                                           &                                                                                                           & 0                                                                                                        &                                                                                                        &                                                                                                        &                                                                                                           &                                                                                                   &                                                                                                         &                                                                                                            &                                                                                                 &                                                                                                &                                                                                                       &                                                                                                       &                                                                                                     &                                                                                                         &                                                                                                             &                                                                                                                                                   \\ 
\hline
Pudding box                                                                                                      &                                                                                                            &                                                                                                        &                                                                                                      &                                                                                                           &                                                                                                           &                                                                                                          & 0                                                                                                      &                                                                                                        &                                                                                                           &                                                                                                   &                                                                                                         &                                                                                                            &                                                                                                 &                                                                                                &                                                                                                       &                                                                                                       &                                                                                                     &                                                                                                         &                                                                                                             &                                                                                                                                                   \\ 
\hline
Gelatin box                                                                                                      &                                                                                                            &                                                                                                        &                                                                                                      &                                                                                                           &                                                                                                           &                                                                                                          &                                                                                                        & 0                                                                                                      &                                                                                                           &                                                                                                   &                                                                                                         &                                                                                                            &                                                                                                 &                                                                                                &                                                                                                       &                                                                                                       &                                                                                                     &                                                                                                         &                                                                                                             &                                                                                                                                                   \\ 
\hline
Potted meat can                                                                                                  &                                                                                                            &                                                                                                        &                                                                                                      &                                                                                                           &                                                                                                           &                                                                                                          &                                                                                                        &                                                                                                        & 0                                                                                                         &                                                                                                   &                                                                                                         &                                                                                                            &                                                                                                 &                                                                                                &                                                                                                       &                                                                                                       &                                                                                                     &                                                                                                         &                                                                                                             &                                                                                                                                                   \\ 
\hline
Banana                                                                                                           &                                                                                                            &                                                                                                        &                                                                                                      &                                                                                                           &                                                                                                           &                                                                                                          &                                                                                                        &                                                                                                        &                                                                                                           & 0                                                                                                 &                                                                                                         &                                                                                                            &                                                                                                 &                                                                                                &                                                                                                       &                                                                                                       &                                                                                                     &                                                                                                         &                                                                                                             &                                                                                                                                                   \\ 
\hline
Pitcher base                                                                                                     &                                                                                                            &                                                                                                        &                                                                                                      &                                                                                                           &                                                                                                           &                                                                                                          &                                                                                                        &                                                                                                        &                                                                                                           &                                                                                                   & 0                                                                                                       &                                                                                                            &                                                                                                 &                                                                                                &                                                                                                       &                                                                                                       &                                                                                                     &                                                                                                         &                                                                                                             &                                                                                                                                                   \\ 
\cline{1-15}\arrayrulecolor{black}\cline{16-16}\arrayrulecolor[rgb]{0.502,0.502,0.502}\cline{17-21}
Bleach cleanser                                                                                                  &                                                                                                            &                                                                                                        &                                                                                                      &                                                                                                           &                                                                                                           &                                                                                                          &                                                                                                        &                                                                                                        &                                                                                                           &                                                                                                   &                                                                                                         & 0                                                                                                          &                                                                                                 &                                                                                                &                                                                                                       &                                                                                                       &                                                                                                     &                                                                                                         &                                                                                                             &                                                                                                                                                   \\ 
\hline
Bowl                                                                                                             &                                                                                                            &                                                                                                        &                                                                                                      &                                                                                                           &                                                                                                           &                                                                                                          &                                                                                                        &                                                                                                        &                                                                                                           &                                                                                                   &                                                                                                         &                                                                                                            & 0                                                                                               &                                                                                                &                                                                                                       &                                                                                                       &                                                                                                     &                                                                                                         &                                                                                                             &                                                                                                                                                   \\ 
\hline
Mug                                                                                                              &                                                                                                            &                                                                                                        &                                                                                                      &                                                                                                           &                                                                                                           &                                                                                                          &                                                                                                        &                                                                                                        &                                                                                                           &                                                                                                   &                                                                                                         &                                                                                                            &                                                                                                 & 0                                                                                              &                                                                                                       &                                                                                                       &                                                                                                     &                                                                                                         &                                                                                                             &                                                                                                                                                   \\ 
\hline
Power drill                                                                                                      &                                                                                                            &                                                                                                        &                                                                                                      &                                                                                                           &                                                                                                           &                                                                                                          &                                                                                                        &                                                                                                        &                                                                                                           &                                                                                                   &                                                                                                         &                                                                                                            &                                                                                                 &                                                                                                & 0                                                                                                     &                                                                                                       &                                                                                                     &                                                                                                         &                                                                                                             &                                                                                                                                                   \\ 
\hline
Wood block                                                                                                       &                                                                                                            &                                                                                                        &                                                                                                      &                                                                                                           &                                                                                                           &                                                                                                          &                                                                                                        &                                                                                                        &                                                                                                           &                                                                                                   &                                                                                                         &                                                                                                            &                                                                                                 &                                                                                                &                                                                                                       & 0                                                                                                     &                                                                                                     &                                                                                                         &                                                                                                             &                                                                                                                                                   \\ 
\hline
Scissors                                                                                                         &                                                                                                            &                                                                                                        &                                                                                                      &                                                                                                           &                                                                                                           &                                                                                                          &                                                                                                        &                                                                                                        &                                                                                                           &                                                                                                   &                                                                                                         &                                                                                                            &                                                                                                 &                                                                                                &                                                                                                       &                                                                                                       & 0                                                                                                   &                                                                                                         &                                                                                                             &                                                                                                                                                   \\ 
\hline
Large marker                                                                                                     &                                                                                                            &                                                                                                        &                                                                                                      &                                                                                                           &                                                                                                           &                                                                                                          &                                                                                                        &                                                                                                        &                                                                                                           &                                                                                                   &                                                                                                         &                                                                                                            &                                                                                                 &                                                                                                &                                                                                                       &                                                                                                       &                                                                                                     & 0                                                                                                       &                                                                                                             &                                                                                                                                                   \\ 
\hline
Extra large clamp                                                                                                &                                                                                                            &                                                                                                        &                                                                                                      &                                                                                                           &                                                                                                           &                                                                                                          &                                                                                                        &                                                                                                        &                                                                                                           &                                                                                                   &                                                                                                         &                                                                                                            &                                                                                                 &                                                                                                &                                                                                                       &                                                                                                       &                                                                                                     &                                                                                                         & 0                                                                                                           &                                                                                                                                                   \\ 
\hline
Foam brick                                                                                                       &                                                                                                            &                                                                                                        &                                                                                                      &                                                                                                           &                                                                                                           &                                                                                                          &                                                                                                        &                                                                                                        &                                                                                                           &                                                                                                   &                                                                                                         &                                                                                                            &                                                                                                 &                                                                                                &                                                                                                       &                                                                                                       &                                                                                                     &                                                                                                         &                                                                                                             & 0                                                                                                                                                 \\
\arrayrulecolor{black}\bottomrule
\end{tabular}
\end{table}

==> tab/procrustes/dist_matrix.tex <==
\renewcommand*\rot[2]{\multicolumn{1}{R{#1}{#2}}}% no optional argument here, please!

% \pgfmathsetmacro\compA{#1/600} %Component R or H
% \pgfmathsetmacro\compB{1} %Component G or S
% \pgfmathsetmacro\compC{1} %Component B or B


%The min, mid and max values
\newcommand*{\MinNumber}{0.0}%
\newcommand*{\MidNumber}{0.2} %
\newcommand*{\MaxNumber}{1.0}%
\def\OmitZero#1.#2.#3!{%
  \ifx\relax#2\relax     % #2 is empty -> no decimal
    #1%
  \else                  % #2 not empty -> decimal
    \ifnum#1=0           % we have 0.
      .#2%
    \else                % we have no 0.xx
      #1.#2%
    \fi
  \fi}

%Apply the gradient macro
\newcommand{\ApplyGradient}[1]{%
    \ifdim #1 pt > \MidNumber pt
    \pgfmathsetmacro{\PercentColor}{max(min(100.0*(#1 - 
    \MidNumber)/(\MaxNumber-\MidNumber),100.0),0.00)} %
    \hspace{-0.33em}\colorbox{green!\PercentColor!red}{\OmitZero#1..!}
    \else
    \pgfmathsetmacro{\PercentColor}{max(min(100.0*(\MidNumber - 
    #1)/(\MidNumber-\MinNumber),100.0),0.00)} %
    \hspace{-0.33em}\colorbox{white!\PercentColor!red}{\OmitZero#1..!}
    \fi
}
\newcolumntype{G}{>{\collectcell\ApplyGradient}c<{\endcollectcell}}
% \renewcommand{\arraystretch}{0}
% \setlength{\fboxsep}{3mm} % box size
% \setlength{\tabcolsep}{0pt}

\begin{table*}[htb]
\centering
\resizebox{\linewidth}{!}{ %< auto-adjusts font size to fill line

\begin{tabular}{r|GGGGGGGGGGGGGGGGGGGG}
&
\rot{45}{1em}{Master chef can} &
\rot{45}{1em}{Cracker box} &
\rot{45}{1em}{Sugar box} &
\rot{45}{1em}{Tomato soup can} &
\rot{45}{1em}{Mustard bottle} &
\rot{45}{1em}{Tuna fish can} &
\rot{45}{1em}{Pudding box} &
\rot{45}{1em}{Gelatin box} &
\rot{45}{1em}{Potted meat can} &
\rot{45}{1em}{Banana} &
\rot{45}{1em}{Pitcher base} &
\rot{45}{1em}{Bleach cleanser} &
\rot{45}{1em}{Bowl} &
\rot{45}{1em}{Mug} &
\rot{45}{1em}{Power drill} &
\rot{45}{1em}{Wood block} &
\rot{45}{1em}{Scissors} &
\rot{45}{1em}{Large marker} &
\rot{45}{1em}{Extra large clamp} &
\rot{45}{1em}{Foam brick}
    \\ \hline
% Master chef can & 0.0000 & 0.1306 & 0.1055 & 0.3591 & 0.1439 & 0.5210 & 0.1797 & 0.3790 & 0.5206 & 0.2407 & 0.9790 & 0.2343 & 0.7408 & 0.5154 & 0.8426 & 0.1165 & 0.3781 & 0.1513 & 0.6862 & 0.5070 \\ 
% Cracker box & 0.1306 & 0.0000 & 0.0700 & 0.5236 & 0.1164 & 0.7482 & 0.2340 & 0.5445 & 0.7308 & 0.1377 & 0.8080 & 0.1545 & 0.5796 & 0.6749 & 0.7802 & 0.1327 & 0.2500 & 0.1692 & 0.5253 & 0.7099 \\ 
% Sugar box & 0.1055 & 0.0700 & 0.0000 & 0.5178 & 0.0518 & 0.6798 & 0.2009 & 0.5518 & 0.6448 & 0.0747 & 0.8286 & 0.0839 & 0.4747 & 0.6235 & 0.5840 & 0.0957 & 0.3111 & 0.1310 & 0.4044 & 0.7067 \\
% Tomato soup can & 0.3591 & 0.5236 & 0.5178 & 0.0000 & 0.5757 & 0.0594 & 0.3922 & 0.0896 & 0.1977 & 0.8041 & 1.6942 & 0.7632 & 0.9517 & 0.2596 & 1.2999 & 0.7376 & 1.0369 & 0.4726 & 1.1395 & 0.0910 \\ 
% Mustard bottle & 0.1439 & 0.1164 & 0.0518 & 0.5757 & 0.0000 & 0.8594 & 0.3175 & 0.6456 & 0.8379 & 0.0725 & 0.7266 & 0.0233 & 0.6891 & 0.7626 & 0.7616 & 0.1541 & 0.2041 & 0.2114 & 0.4915 & 0.8681 \\ 
% Tuna fish can & 0.5210 & 0.7482 & 0.6798 & 0.0594 & 0.8594 & 0.0000 & 0.2677 & 0.0809 & 0.0766 & 0.8343 & 1.7471 & 1.0391 & 0.9073 & 0.1315 & 1.1260 & 0.6276 & \textbf{1.1393} & 0.4115 & 1.2167 & 0.0286 \\ 
% Pudding box & 0.1797 & 0.2340 & 0.2009 & 0.3922 & 0.3175 & 0.2677 & 0.0000 & 0.3542 & 0.1921 & 0.3368 & 1.1653 & 0.4212 & 0.7149 & 0.2212 & 0.8810 & 0.2033 & 0.5049 & 0.0728 & 0.7097 & 0.2824 \\ 
% Gelatin box & 0.3790 & 0.5445 & 0.5518 & 0.0896 & 0.6456 & 0.0809 & 0.3542 & 0.0000 & 0.1666 & \textbf{0.8923} & \textbf{1.7623} & 0.7978 & \textbf{1.0369} & 0.1696 & \textbf{1.2846} & 0.6858 & 1.0249 & 0.4616 & 1.0467 & 0.0721 \\ 
% Potted meat can & 0.5206 & 0.7308 & 0.6448 & 0.1977 & 0.8379 & 0.0766 & 0.1921 & 0.1666 & 0.0000 & 0.8824 & 1.5991 & 0.9827 & 0.8007 & 0.1085 & 1.0595 & 0.5961 & 1.0283 & 0.3960 & 0.9701 & 0.1254 \\ 
% Banana & 0.2407 & 0.1377 & 0.0747 & 0.8041 & 0.0725 & 0.8343 & 0.3368 & 0.8923 & 0.8824 & 0.0000 & 0.6522 & 0.0760 & 0.5416 & 0.8215 & 0.6225 & 0.1395 & 0.1833 & 0.2097 & 0.4222 & 0.8484 \\ 
% Pitcher base & \textbf{0.9790} & \textbf{0.8080} & \textbf{0.8286} & \textbf{1.6942} & 0.7266 & \textbf{1.7471} & \textbf{1.1653} & \textbf{1.7623} & \textbf{1.5991} & 0.6522 & 0.0000 & 0.6146 & 0.5397 & \textbf{1.4022} & 0.3933 & \textbf{0.7589} & 0.4715 & \textbf{1.0331} & 0.3980 & 1.6402 \\ 
% Bleach cleanser & 0.2343 & 0.1545 & 0.0839 & 0.7632 & 0.0233 & 1.0391 & 0.4212 & 0.7978 & 0.9827 & 0.0760 & 0.6146 & 0.0000 & 0.6863 & 0.8838 & 0.7086 & 0.1643 & 0.1870 & 0.2882 & 0.4266 & 1.0751 \\ 
% Bowl & 0.7408 & 0.5796 & 0.4747 & 0.9517 & 0.6891 & 0.9073 & 0.7149 & 1.0369 & 0.8007 & 0.5416 & 0.5397 & 0.6863 & 0.0000 & 0.8730 & 0.1506 & 0.6438 & 0.2759 & 0.5808 & 0.1865 & 0.9340 \\ 
% Mug & 0.5154 & 0.6749 & 0.6235 & 0.2596 & 0.7626 & 0.1315 & 0.2212 & 0.1696 & 0.1085 & 0.8215 & 1.4022 & 0.8838 & 0.8730 & 0.0000 & 1.1381 & 0.5355 & 0.9293 & 0.3541 & 1.0989 & 0.1263 \\ 
% Power drill & 0.8426 & 0.7802 & 0.5840 & 1.2999 & 0.7616 & 1.1260 & 0.8810 & 1.2846 & 1.0595 & 0.6225 & 0.3933 & 0.7086 & 0.1506 & 1.1381 & 0.0000 & 0.5908 & 0.3160 & 0.7392 & 0.1716 & 1.1663 \\ 
% Wood block & 0.1165 & 0.1327 & 0.0957 & 0.7376 & 0.1541 & 0.6276 & 0.2033 & 0.6858 & 0.5961 & 0.1395 & 0.7589 & 0.1643 & 0.6438 & 0.5355 & 0.5908 & 0.0000 & 0.2609 & 0.1451 & 0.5787 & 0.6275 \\ 
% Scissors & 0.3781 & 0.2500 & 0.3111 & 1.0369 & 0.2041 & 1.1393 & 0.5049 & 1.0249 & 1.0283 & 0.1833 & 0.4715 & 0.1870 & 0.2759 & 0.9293 & 0.3160 & 0.2609 & 0.0000 & 0.3609 & 0.1221 & 1.1219 \\ 
% Large marker & 0.1513 & 0.1692 & 0.1310 & 0.4726 & 0.2114 & 0.4115 & 0.0728 & 0.4616 & 0.3960 & 0.2097 & 1.0331 & 0.2882 & 0.5808 & 0.3541 & 0.7392 & 0.1451 & 0.3609 & 0.0000 & 0.6270 & 0.4066 \\ 
% Extra large clamp & 0.6862 & 0.5253 & 0.4044 & 1.1395 & 0.4915 & 1.2167 & 0.7097 & 1.0467 & 0.9701 & 0.4222 & 0.3980 & 0.4266 & 0.1865 & 1.0989 & 0.1716 & 0.5787 & 0.1221 & 0.6270 & 0.0000 & \textbf{1.2884} \\ 
% Foam brick & 0.5070 & 0.7099 & 0.7067 & 0.0910 & \textbf{0.8681} & 0.0286 & 0.2824 & 0.0721 & 0.1254 & 0.8484 & 1.6402 & \textbf{1.0751} & 0.9340 & 0.1263 & 1.1663 & 0.6275 & 1.1219 & 0.4066 & \textbf{1.2884} & 0.0000 \\ \hline
Master chef can & 0.00 & 0.07 & 0.06 & 0.20 & 0.08 & 0.30 & 0.10 & 0.22 & 0.30 & 0.14 & 0.56 & 0.13 & 0.42 & 0.29 & 0.48 & 0.07 & 0.21 & 0.09 & 0.39 & 0.29 \\
Cracker box & 0.07 & 0.00 & 0.04 & 0.30 & 0.07 & 0.42 & 0.13 & 0.31 & 0.41 & 0.08 & 0.46 & 0.09 & 0.33 & 0.38 & 0.44 & 0.08 & 0.14 & 0.10 & 0.30 & 0.40 \\
Sugar box & 0.06 & 0.04 & 0.00 & 0.29 & 0.03 & 0.39 & 0.11 & 0.31 & 0.37 & 0.04 & 0.47 & 0.05 & 0.27 & 0.35 & 0.33 & 0.05 & 0.18 & 0.07 & 0.23 & 0.40 \\
Tomato soup can & 0.20 & 0.30 & 0.29 & 0.00 & 0.33 & 0.03 & 0.22 & 0.05 & 0.11 & 0.46 & 0.96 & 0.43 & 0.54 & 0.15 & 0.74 & 0.42 & 0.59 & 0.27 & 0.65 & 0.05 \\
Mustard bottle & 0.08 & 0.07 & 0.03 & 0.33 & 0.00 & 0.49 & 0.18 & 0.37 & 0.48 & 0.04 & 0.41 & 0.01 & 0.39 & 0.43 & 0.43 & 0.09 & 0.12 & 0.12 & 0.28 & 0.49 \\
Tuna fish can & 0.30 & 0.42 & 0.39 & 0.03 & 0.49 & 0.00 & 0.15 & 0.05 & 0.04 & 0.47 & 0.99 & 0.59 & 0.51 & 0.07 & 0.64 & 0.36 & 0.65 & 0.23 & 0.69 & 0.02 \\
Pudding box & 0.10 & 0.13 & 0.11 & 0.22 & 0.18 & 0.15 & 0.00 & 0.20 & 0.11 & 0.19 & 0.66 & 0.24 & 0.41 & 0.13 & 0.50 & 0.12 & 0.29 & 0.04 & 0.40 & 0.16 \\
Gelatin box & 0.22 & 0.31 & 0.31 & 0.05 & 0.37 & 0.05 & 0.20 & 0.00 & 0.09 & 0.51 & 1.00 & 0.45 & 0.59 & 0.10 & 0.73 & 0.39 & 0.58 & 0.26 & 0.59 & 0.04 \\
Potted meat can & 0.30 & 0.41 & 0.37 & 0.11 & 0.48 & 0.04 & 0.11 & 0.09 & 0.00 & 0.50 & 0.91 & 0.56 & 0.45 & 0.06 & 0.60 & 0.34 & 0.58 & 0.22 & 0.55 & 0.07 \\
Banana & 0.14 & 0.08 & 0.04 & 0.46 & 0.04 & 0.47 & 0.19 & 0.51 & 0.50 & 0.00 & 0.37 & 0.04 & 0.31 & 0.47 & 0.35 & 0.08 & 0.10 & 0.12 & 0.24 & 0.48 \\
Pitcher base & 0.56 & 0.46 & 0.47 & 0.96 & 0.41 & 0.99 & 0.66 & 1.00 & 0.91 & 0.37 & 0.00 & 0.35 & 0.31 & 0.80 & 0.22 & 0.43 & 0.27 & 0.59 & 0.23 & 0.93 \\
Bleach cleanser & 0.13 & 0.09 & 0.05 & 0.43 & 0.01 & 0.59 & 0.24 & 0.45 & 0.56 & 0.04 & 0.35 & 0.00 & 0.39 & 0.50 & 0.40 & 0.09 & 0.11 & 0.16 & 0.24 & 0.61 \\
Bowl & 0.42 & 0.33 & 0.27 & 0.54 & 0.39 & 0.51 & 0.41 & 0.59 & 0.45 & 0.31 & 0.31 & 0.39 & 0.00 & 0.50 & 0.09 & 0.37 & 0.16 & 0.33 & 0.11 & 0.53 \\
Mug & 0.29 & 0.38 & 0.35 & 0.15 & 0.43 & 0.07 & 0.13 & 0.10 & 0.06 & 0.47 & 0.80 & 0.50 & 0.50 & 0.00 & 0.65 & 0.30 & 0.53 & 0.20 & 0.62 & 0.07 \\
Power drill & 0.48 & 0.44 & 0.33 & 0.74 & 0.43 & 0.64 & 0.50 & 0.73 & 0.60 & 0.35 & 0.22 & 0.40 & 0.09 & 0.65 & 0.00 & 0.34 & 0.18 & 0.42 & 0.10 & 0.66 \\
Wood block & 0.07 & 0.08 & 0.05 & 0.42 & 0.09 & 0.36 & 0.12 & 0.39 & 0.34 & 0.08 & 0.43 & 0.09 & 0.37 & 0.30 & 0.34 & 0.00 & 0.15 & 0.08 & 0.33 & 0.36 \\
Scissors & 0.21 & 0.14 & 0.18 & 0.59 & 0.12 & 0.65 & 0.29 & 0.58 & 0.58 & 0.10 & 0.27 & 0.11 & 0.16 & 0.53 & 0.18 & 0.15 & 0.00 & 0.20 & 0.07 & 0.64 \\
Large marker & 0.09 & 0.10 & 0.07 & 0.27 & 0.12 & 0.23 & 0.04 & 0.26 & 0.22 & 0.12 & 0.59 & 0.16 & 0.33 & 0.20 & 0.42 & 0.08 & 0.20 & 0.00 & 0.36 & 0.23 \\
Extra large clamp & 0.39 & 0.30 & 0.23 & 0.65 & 0.28 & 0.69 & 0.40 & 0.59 & 0.55 & 0.24 & 0.23 & 0.24 & 0.11 & 0.62 & 0.10 & 0.33 & 0.07 & 0.36 & 0.00 & 0.73 \\
Foam brick & 0.29 & 0.40 & 0.40 & 0.05 & 0.49 & 0.02 & 0.16 & 0.04 & 0.07 & 0.48 & 0.93 & 0.61 & 0.53 & 0.07 & 0.66 & 0.36 & 0.64 & 0.23 & 0.73 & 0.00 \\ \hline
\end{tabular}

} % \resizebox
\caption{
% 
\textbf{Distance matrix of mean hand shapes (best seen in colour)} -- Normalised Procrustes distances of mean hand shapes for
each object. Column-wise highest distances tend towards green. The \textit{Pitcher base} is the object inducing the most different grasps in the dataset.
% 
} % \caption
\label{tab:dist_mat}
\end{table*}


==> tab/procrustes/dist_matrix_2.tex <==
\begingroup
    \renewcommand*{\arraystretch}{1.5}%
    \newcommand*{\headformat}[1]{{\small#1}}%
    \newcommand*{\vcorr}{%
      \vadjust{\vspace{-\dp\csname @arstrutbox\endcsname}}%
      \global\let\vcorr\relax
    }%
    \newcommand*{\HeadAux}[1]{%
      \multicolumn{1}{@{}r@{}}{%
        \vcorr
        \sbox0{\headformat{\strut #1}}%
        \sbox2{\headformat{Complex Data Movement}}%
        \sbox4{\kern\tabcolsep\redtriangle\kern\tabcolsep}%
        \sbox6{\rotatebox{45}{\rule{0pt}{\dimexpr\ht0+\dp0\relax}}}%
        \sbox0{\raisebox{.5\dimexpr\dp0-\ht0\relax}[0pt][0pt]{\unhcopy0}}%
        \kern.75\wd4 %
        \rlap{%
          \raisebox{.25\wd4}{\rotatebox{45}{\unhcopy0}}%
        }%
        \kern.25\wd4 %
        \ifx\HeadLine Y%
          \dimen0=\dimexpr\wd2+.5\wd4\relax
          \rlap{\rotatebox{45}{\hbox{\vrule width\dimen0 height .4pt}}}%
        \fi
      }%
    }%
    \newcommand*{\head}[1]{\HeadAux{\global\let\HeadLine=Y#1}}%
    \newcommand*{\headNoLine}[1]{\HeadAux{\global\let\HeadLine=N#1}}%
    \noindent
    \begin{tabular}{%
      >{\bfseries}lc|>{\quad}c
      *{4}{c|}c>{\quad}c
      *{4}{c|}c>{\quad}c
      *{2}{c|}c%
    }%
      &
      \head{master\_chef\_can} &
      \head{cracker\_box} &
      \head{sugar\_box} &
      \head{tomato\_soup\_can} &
      \head{mustard\_bottle} &
      \head{tuna\_fish\_can} &
      \head{pudding\_box} &
      \head{gelatin\_box} &
      \head{potted\_meat\_can} &
      \head{banana} &
      \head{pitcher\_base} &
      \head{bleach\_cleanser} &
      \head{bowl} &
      \head{mug} &
      \head{power\_drill} &
      \head{wood\_block} &
      \head{scissors} &
      \head{large\_marker} &
      \head{extra\_large\_clamp} &
      \head{foam\_brick} &
      \\
      \sbox0{S}%
      \rule{0pt}{\dimexpr\ht0 + 2ex\relax}%
      master\_chef\_can &  &&
       &  & & & &&
       &  & & & &&
       &  & 
      \\\hline
       cracker\_box &  &&
       &  & & & &&
       &  & & & &&
       &  & 
      \\\hline
       sugar\_box &  &&
       &  & & & &&
       &  & & & &&
       &  & 
      \\\hline
       tomato\_soup\_can &  &&
       &  & & & &&
       &  & & & &&
       &  & 
      \\\hline
       mustard\_bottle &  &&
       &  & & & &&
       &  & & & &&
       &  & 
      \\\hline
      tuna\_fish\_can &  &&
       &  & & & &&
       &  & & & &&
       &  & 
      \\\hline
      pudding\_box &  &&
      & & & & &&
      & & & & &&
      & &
      \\\hline
      gelatin\_box &  &&
      & & & & &&
      & & & & &&
      & & 
      \\\hline
      potted\_meat\_can &  &&
      & & & & &&
      & & & & &&
      & & 
      \\\hline
      banana &  &&
      & & & & &&
      & & & & &&
      & &
      \\\hline
      pitcher\_base &  &&
      & & & & &&
      & & & & &&
      & &
      \\\hline
      bleach\_cleanser &  &&
      & & & & &&
      & & & & &&
      & &
      \\\hline
     bowl &  &&
      & & & & &&
      & & & &
        &&
      & & 
      \\\hline
     mug &  &&
      & & & & &&
      & & & &
        &&
      & & 
      \\\hline
     power\_drill &  &&
      & & & & &&
      & & & &
        &&
      & & 
      \\\hline
     wood\_block &  &&
      & & & & &&
      & & & &
        &&
      & & 
      \\\hline
     scissors &  &&
      & & & & &&
      & & & &
        &&
      & & 
      \\\hline
     large\_marker &  &&
      & & & & &&
      & & & &
        &&
      & & 
      \\\hline
     extra\_large\_clamp &  &&
      & & & & &&
      & & & &
        &&
      & & 
      \\\hline
     foam\_brick &  &&
      & & & & &&
      & & & &
        &&
      & & 
      \\
    \end{tabular}%
    \kern19.5mm % manually with the help of the next \vrule
    % \vrule height 50mm
  \endgroup
